Around Average Behavior: 3-lambda Network Model

The analysis of networks affects the research of many real phenomena. The complex network structure can be viewed as a network's state at the time of the analysis or as a result of the process through which the network arises. Research activities focus on both and, thanks to them, we know not only many measurable properties of networks but also the essence of some phenomena that occur during the evolution of networks. One typical research area is the analysis of co-authorship networks and their evolution. In our paper, the analysis of one real-world co-authorship network and inspiration from existing models form the basis of the hypothesis from which we derive new 3-lambda network model. This hypothesis works with the assumption that regular behavior of nodes revolves around an average. However, some anomalies may occur. The 3-lambda model is stochastic and uses the three parameters associated with the average behavior of the nodes. The growth of the network based on this model assumes that one step of the growth is an interaction in which both new and existing nodes are participating. In the paper we present the results of the analysis of a co-authorship network and formulate a hypothesis and a model based on this hypothesis. Later in the paper, we examine the outputs from the network generator based on the 3-lambda model and show that generated networks have characteristics known from the environment of real-world networks.

==> Arxiv latex submitted/dblp.tex <==
\section{DBLP Dataset Analysis} 
\label{sec:dblp}

We studied the DBLP dataset which contains basic bibliographic information of publications from the computer science field. This data is freely available\footnote{\url{http://www.informatik.uni-trier.de/~ley/db/}} and contains highly relevant information about publication activity from the period of nearly fifty years, even though they are not complete. At the time we downloaded this dataset (July 2016), and after first pre-processing, it contained a total of $2988015$ publications. Further characteristics can be seen in Table \ref{tab:dblp}. 
\begin{table}[htbp]
  \centering
  \caption{DBLP dataset}
    \begin{tabular}{|l|r|} 
		\hline
    Total number of publications & 2988015 \\
    Total number of authors & 1622828 \\
    Mean papers per author & 5.113 \\
    Mean authors per paper & 2.895 \\
    \hline
    \end{tabular}%
  \label{tab:dblp}%
\end{table}%

Based on the co-authorship of authors, we constructed a social network where authors are linked if they co-authored a paper. The weight of the edge corresponds to the number of co-authored papers. Basic characteristics of this network and its maximal connected component are in Table \ref{tab:dblpcompo}.


\begin{table}[htbp]
  \centering
  \caption{DBLP network and its max. connected component}
	%\resizebox{0.8\columnwidth}{!}{
		\begin{tabular}{|l|rr|}
    \hline
          & $net$ & $max CC$\\
    \hline
    Total number of nodes & 1554772 & 1408331 \\
    Total number of edges & 6930545 & 6768108 \\
    Density & 5.73\mbox{\sc{e}-}06 & 6.83\mbox{\sc{e}-}06 \\
    Mean degree & 8.915 & 9.612 \\
    Number of connected components & 49459 & 1 \\
    Global clustering coefficient & 0.1749 & 0.1741 \\
    Mean local cluster coefficient & 0.7341 & 0.7217 \\
    Mean edge weight & 1.746 & 1.762 \\
    Number of communities (Louvain) &   -    & 422 \\
    \hline
    \end{tabular}%
		%}
  \label{tab:dblpcompo}%
\end{table}%

In additional pre-processing of the dataset, we set each publication a month which corresponded to the date of a conference or date of publication in a journal, respectively.  If the record in the DBPL did not contain the month of publication, we chose the month for a given year randomly. Furthermore, we assumed that the author existing in a given month is the author who had at least one publication in the month preceding the given month. In the next step, we dropped all publications that did not contain any already existing authors. For the rest of publications, we have identified the main author, who was the first existing author in the order of the co-authors of these publications.


The first objective of the experiment with the DBLP dataset was to discover what shape has the distribution of the number of publications depending on the number of co-authors of the main author. Figure \ref{fig:poisfit} shows the distribution for the first twenty values (i.e. up to $20$ co-authors) and cumulative distribution of all values (except for one publication with $286$ authors). This distribution is compared to a Poisson distribution with a $\lambda$ value equal to the average number of co-authors, which is $1.99$.


\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{figures/poisfit}
  \caption{DBLP: Poisson distribution}\label{fig:poisfit}
\end{figure}

The second objective of the experiment was to find authors who are most often in the role of the main author of a publication. The results of this part of the experiment are to be understood only as an estimate based on the above-mentioned assumptions about the main author. Empirical distribution, together with the theoretical value of the Poisson distribution for the first fifteen authors with the highest number of publications in the role of the first author, is shown in Figure \ref{fig:top15}.

\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{figures/proactive_coauthors_top15}
  \caption{Co-authors histograms for top 15 authors (by number of publications)}
	\label{fig:top15}
\end{figure}

\subsection{Hypothesis}
Results of the analysis of the DBLP dataset can not be easily generalized. However, experiments have shown quite clearly that the probability of a publication with a certain number of co-authors follows the Poisson distribution. If we extend thoughts about the main author by what kind and how many different co-authors he/she has, we may divide co-authors into three groups. In the first group are authors with whom the main author has previously published. In the second group are those who have previously published but not yet together with the main author. In the third group are new authors, i.e. those who have no previous publications. We can then formulate a hypothesis, based on which we define the new network model in the next part of the paper.

\bigbreak
\textbf{Hypothesis}
\begin{enumerate}
	\item The variables describing the number of co-authors in different groups are independent random variables.
  \item Just as the total number of co-authors, these variables follow Poisson distribution.
\end{enumerate}

In this paper, we are working with a co-authorship network, which is essentially a collaborative network. Therefore, the presented model can not be taken as a universal model. The model is primarily about a simple simulation of the development of collaborative networks inspired by analyzing the co-authorship network.


==> Arxiv latex submitted/experiment.tex <==
\section{Experimental Evaluation}
\label{sec:exp}
We are using using three different settings, $Setting = [\lambda_1, \lambda_2, \lambda_3]$, in the experiments. In $Setting_1 = [1.6, 0.35, 0.05]$, the average interaction involved three nodes (a triad), which corresponds approximately to the analyzed co-authorship network. This setting presumes the interaction is dominated by neighbors of the proactive node with the occasional participation of new nodes and rather exceptional participation of existing nodes yet not connected to the proactive node. In $Setting_2 = [3, 6, 1]$ predominate new nodes, and the average number of nodes in interaction is $11$. In $Setting_3 = [0.45, 0.45, 0.1]$ interaction involved two nodes (a dyad) on average, wherein the number of neighbors and new nodes are balanced and new connection occurrences are less likely.

\begin{figure}[ht]
	\centering
  \begin{subfigure}{2.7cm}
    \centering\includegraphics[width=2.5cm]{figures/distr_stupnu_Setting1}
    \caption{$Setting_1$}
  \end{subfigure}
  \begin{subfigure}{2.7cm}
    \centering\includegraphics[width=2.5cm]{figures/distr_stupnu_Setting2}
    \caption{$Setting_2$}
		  \end{subfigure}
   \begin{subfigure}{2.7cm}
    \centering\includegraphics[width=2.5cm]{figures/distr_stupnu_Setting3}
    \caption{$Setting_3$}
  \end{subfigure}
	\caption{Degree distribution}
\label{fig:DD}
\end{figure}

\begin{figure}[ht]
	\centering
  \begin{subfigure}{2.7cm}
    \centering\includegraphics[width=2.5cm]{figures/inter_per_vert_Setting1}
    \caption{$Setting_1$}
  \end{subfigure}
  \begin{subfigure}{2.7cm}
    \centering\includegraphics[width=2.5cm]{figures/inter_per_vert_Setting2}
    \caption{$Setting_2$}
		  \end{subfigure}
   \begin{subfigure}{2.7cm}
    \centering\includegraphics[width=2.5cm]{figures/inter_per_vert_Setting3}
    \caption{$Setting_3$}
  \end{subfigure}
	\caption{Interactions per	node}
\label{fig:IpN}
\end{figure}

\begin{figure}[ht]
	\centering
  \begin{subfigure}{2.7cm}
    \centering\includegraphics[width=2.5cm]{figures/dist_vel_komf_Setting1}
    \caption{$Setting_1$}
  \end{subfigure}
  \begin{subfigure}{2.7cm}
    \centering\includegraphics[width=2.5cm]{figures/dist_vel_komf_Setting2}
    \caption{$Setting_2$}
		  \end{subfigure}
   \begin{subfigure}{2.7cm}
    \centering\includegraphics[width=2.5cm]{figures/dist_vel_komf_Setting3}
    \caption{$Setting_3$}
  \end{subfigure}
	\caption{Community size}
\label{fig:ComSize}
\end{figure}


\subsection{Properties of Generated Network}

\begin{table*}[ht]
  \centering
  \caption{Global properties}
		\begin{tabular}{|c|r|rrrrrrrrrrr|}
\hline
Setting &  & $n$ & $m$ & $<$k$>$ &  $<$l$>$ & $l_{max}$ & $CC$ & $r$ & $com_{IM}$ & $com_L$ & $Q_{IM}$ & $Q_L$ \\ 
\hline
$Setting_1$ & mean & 10001.10 & 40108.97 & 8.0209 & 4.8101 & 12.07 & 0.6555 & 0.14522 & 609.40 & 54.70 & 0.6424 & 0.7119 \\ 
& sd & 0.31 & 398.80 & 0.0797 & 0.0421 & 0.64 & 0.0029 & 0.01769 & 12.37 & 7.04 & 0.0062 & 0.0085 \\ 
\hline	
$Setting_2$ & mean & 10003.87 & 88620.40 & 17.7172 & 4.2369 & 8.43  & 0.8087 & 0.12961 & 422.60 & 42.90 & 0.6772 & 0.7334 \\ 
& sd & 1.53 & 797.95 & 0.1600 & 0.0277 & 0.63  & 0.0018 & 0.00913 & 10.30 & 2.78 & 0.0049 & 0.0067 \\ 
\hline
$Setting_3$ & mean & 10001.17 & 21494.57 & 4.2984 & 6.8965 & 16.23 & 0.4784 & 0.19907 & 953.30 & 68.70 & 0.7276 & 0.8129 \\ 
&  sd & 0.46 & 142.64 & 0.0285 & 0.0609 & 0.63 & 0.0044 & 0.01222 & 15.55 & 3.19 & 0.0035 & 0.0038 \\ 
\hline
\end{tabular}%
  \label{tab:gp}%
\end{table*}%
\begin{table}[ht]
  \centering
  \caption{Interactions}
\begin{tabular}{|r|r|rrr|}
	\hline
Setting & & $I$ & $<$i$>$ & $<$s$>$ \\ 
\hline
$Setting_1$ & mean & 28561.90 & 8.0887 & 2.8323 \\ 
&  sd & 278.93 & 0.0817 & 0.0082 \\ 
\hline	
$Setting_2$ & mean & 1664.53 & 1.8278 & 10.9860 \\ 
& sd & 17.69 & 0.0115 & 0.0824 \\
\hline	
$Setting_3$ & mean & 22204.43 & 4.3772 & 1.9716 \\ 
& sd & 202.06 & 0.0292 & 0.0069 \\ 
\hline
	\end{tabular}%
  \label{tab:interact}%
\end{table}%

In the first experiment, we show the properties of networks generated with different settings. We generated for each setting $100$ networks with approximately $10000$ nodes. Table \ref{tab:gp} summarizes average values (and standard deviation) of measured properties for each setting. Measured properties include number of nodes $n$ and edges $m$, average degree $<$k$>$, average shortest path length $<$l$>$, diameter $L_{max}$, average clustering coefficient $CC$, assortativity $r$, number of communities detected by Infomap \cite{rosvall2009map} $com_{IM}$ and Louvain \cite{blondel2008fast} $com_L$ algorithm, and corresponding modularities $Q_{IM}$ and $Q_L$, respectively. Table \ref{tab:interact} contains average values associated with the temporality of the network, i.e. total number of interactions $I$, average number of interactions $<$i$>$ and average number of nodes in interaction $<$s$>$. Figures \ref{fig:DD}-\ref{fig:ComSize} show degree distribution, number of interactions distribution and distributions of community size detected by Infomap algorithm.

The experiment indicates that all three settings generate networks with small-world and scale-free characteristics. The first and second setting have generated networks of high average clustering coefficient. Networks have a tendency to be assortative. Assortativity values correspond to all settings to the values known from social networks \cite{newman2002assortative}. Generated networks also have community structure and a high modularity for all settings.

\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{figures/setting1_1000}
  \caption{Network: 1000 nodes, $Setting_1$}
	\label{fig:Set1000}
\end{figure}

Figure \ref{fig:Set1000} shows a network with $1000$ nodes and $3599$ edges generated with $Setting_1$. A total of $2830$ interactions took place. The size of nodes and strength of edges correspond to the number of interactions they took part in, the labels indicate the order in which nodes were created. The network has an overlapping community and core-periphery structure. Colored 19 communities were detected by Louvain method, modularity is $0.746$.

\subsection{Evolution of Generated Network}
The subject of the second experiment is one network generated with $Setting_1$. The aim is to show the development of network properties during its growth. The values for each characteristic are measured when the network has $10, 20, 50, 100$, ..., and $10000$ nodes. The results are summarized in Table \ref{tab:Evolut}.

\begin{table*}[ht]
  \centering
  \caption{Evolution of network properties}
	\begin{tabular}{|r|rrrrrrrrrr|}

\hline
  $n$ & $m$ & $<$k$>$ &  $<$l$>$ & $l_{max}$ & $CC$ & $r$ & $com_{IM}$ & $com_L$ & $Q_{IM}$ & $Q_L$ \\
\hline
  10 & 27.00 & 5.4000 & 1.4000 & 20 & 0.8195 & -0.41738 & 1 & 3 & 0.0000 & 0.0590 \\ 
 20 & 53.00 & 5.3000 & 2.0684 & 5 & 0.5804 & -0.09355 & 2 & 4 & 0.0361 & 0.2398 \\ 
  50 & 184.00 & 7.3600 & 2.5004 & 7 & 0.6248 & -0.00886 & 5 & 5 & 0.2957 & 0.3742 \\ 
100 & 388.00 & 7.7600 & 2.8731 & 6 & 0.6793 & 0.09177 & 11 & 9 & 0.4259 & 0.4613 \\ 
 200 & 812.00 & 8.1200 & 3.1859 & 7 & 0.6824 & 0.05107 & 20 & 11 & 0.5002 & 0.5121 \\ 
500 & 2112.00 & 8.4480 & 3.6095 & 8 & 0.6394 & 0.11911 & 44 & 11 & 0.5540 & 0.5849 \\ 
 1000 & 4053.00 & 8.1060 & 3.9402 & 9 & 0.6592 & 0.14528 & 83 & 17 & 0.5812 & 0.6341 \\ 
2000 & 8306.00 & 8.3060 & 4.2054 & 10 & 0.6538 & 0.14016 & 151 & 24 & 0.5972 & 0.6714 \\ 
5000 & 20316.00 & 8.1264 & 4.5344 & 12 & 0.6603 & 0.15823 & 342 & 44 & 0.6203 & 0.6827 \\ 
10000 & 40476.00 & 8.0952 & 4.8015 & 11 & 0.6557 & 0.15351 & 645 & 64 & 0.6307 & 0.7003 \\ 
\hline
  \end{tabular}
	  \label{tab:Evolut}%
\end{table*}%
	
Figure \ref{fig:EvolNet}, similarly to the previous experiment, shows the distribution of degree, number of interactions and size of communities. The evolution of these properties is portrayed when network has $100, 200, 1000, 5000, 10000$ nodes.

\begin{figure*}[ht]
\centering
\includegraphics[width=46em]{figures/distribution_10_20_50}
\caption{Evolution of network (100, 200, 1000, 5000, 10000 nodes)}
\label{fig:EvolNet}
\end{figure*}

Key properties (average degree, shortest path, clustering coefficient, assortativity, modularity) happen to stabilize their values between $1000$ and $10000$ nodes. Our experiments show that  generated networks with other settings also have similar behavior. Figure \ref{fig:InterEvol} shows the evolution of the number of interactions for fifteen nodes with the highest number of interactions at the end of the generation process. The ID of a node represents the moment of its creation. The trend shows how the chances of participating in interactions increase for nodes that already have a high number of interactions.

\begin{figure}[ht]
\centering
\includegraphics[width =\linewidth]{figures/Interaction_evolution}
\caption{Evolution of nodes with the most interactions}
\label{fig:InterEvol}
\end{figure}


\subsection{Correlations}
In this experiment, we compare the analyzed real-world network with generated networks. For each setting we generated a network with one million nodes. Then we examined the correlation between the node's creation time and it's degree and number of interactions, respectively. The emergence of the node is represented by its $ID$, which is in the order of its creation. Furthermore, we calculated the correlation between degree and number of node's interactions. We did the same for the analyzed DBLP dataset, where the order of nodes is to be understood as an estimate based on data pre-processing described in Section \ref{sec:dblp}.

\begin{table}[ht]
  \centering
  \caption{Correlations}
\begin{tabular}{|r|rrr|}
	\hline
Setting & $\rho(Id, k)$ & $\rho(Id, i)$ & $\rho(k, i)$ \\ 
\hline
$Setting_1$ & -0.59 & -0.50 & 0.96 \\  
\hline	
$Setting_2$ & -0.47 & -0.47 & 0.95 \\ 
\hline	
$Setting_3$ & -0.70 & -0.58 & 0.87 \\ 
\hline
DBLP & -0.23 & -0.18 & 0.84 \\ 
\hline
	\end{tabular}%
  \label{tab:corr}%
\end{table}%

The results summarized in Table \ref{tab:corr} show that regardless of the setting, the first two correlations are much higher in the 3-lambda model than in the DBLP dataset (Pearson's correlation coefficient was used). Thus, in the presented model, older nodes have a higher (and continuous) chance to participate in interactions than in reality. The cause is probably the aging of nodes in real-world networks where nodes, at different times, no longer participate in interactions. This significantly affects the evolution (growth) and some properties of the network.

Previous experiments demonstrated that despite the absence of aging, generated networks have very good properties. We have not, therefore, for reasons of simplicity, incorporated any of the known models of aging (e.g. inspired by \cite{dorogovtsev2000evolution, xu2010evolutionary}) to the 3-lambda network model.

==> Arxiv latex submitted/model.tex <==
\section{3-lambda Model} 
\label{sec:met}
%As mentioned in the introduction, the model is based on the assumption that one-step of the network's growth is one interaction. Both new and existing nodes are involved in the interaction and after the interaction there are edges between all involved pairs of nodes. Some (or all) of these edges between pairs of involved nodes could exist before the interaction. The model is inherently temporal, since with each node or edge we can associate the list of interactions in which they participated during the growth of the network (list of interactions is a list of steps of the growth in the order in which interactions took place). It is further assumed that neither nodes nor edges age, so they are not removed during the growth of the network. From this perspective, the model is growing.

\begin{figure*}[ht]
\centering
 \begin{subfigure}{17em}
  \centering
	\includegraphics[width = 16em]{figures/200-0-3-0}
\caption{$\lambda_1$ = 0, $\lambda_2$ = 3, $\lambda_3$ = 0}
\label{fig:lambda2net}
 \end{subfigure}
 \begin{subfigure}{17em}
	\centering
		\includegraphics[width =16em]{figures/200-2-3-0}
		\caption{$\lambda_1$ = 2, $\lambda_2$ = 3, $\lambda_3$ = 0}
		\label{fig:lambda1net}
  \end{subfigure}
  \begin{subfigure}[ht]{17em}
		\centering
			\includegraphics[width =16em]{figures/200-2-3-05}
			\caption{$\lambda_1$ = 2, $\lambda_2$ = 3, $\lambda_3$ = 0.5}
			\label{fig:lambda3net}
  \end{subfigure}
	\caption{3-lambda model: generated networks with $200$ nodes}
\label{fig:L3D}
\end{figure*}

As mentioned in the introduction, the model is based on the assumption that one step of the network's growth is one interaction. Both new and existing nodes are involved in the interaction, and after the interaction, there are edges between all involved pairs of nodes. Some (or all) of these edges between pairs of involved nodes could exist before the interaction. The model is inherently temporal since we can associate with each node or edge the list of interactions in which they participated during the growth of the network (the list of interactions is a list of steps of the growth in the order in which the interactions took place). It is further assumed that neither nodes nor edges age, so they are not removed during the growth of the network. From this perspective the model is growing.

In the model, nodes involved in the interaction have four different roles:

\begin{enumerate}
	\item key node of the interaction (proactive)
  \item nodes adjacent to the proactive node (neighbors)
  \item new nodes (newbies)
  \item nodes that are not adjacent to the proactive node (new connections)
\end{enumerate}

It is essential for the model that each interaction always contains exactly one proactive node and may (but doesn't have to) include nodes in three other roles. How many spots will be represented by each of these three roles is selected based on the Poisson distribution with a preselected $\lambda_1$ (neighbors); $\lambda_2$ (newbies); and $\lambda_3$ (new connections). Furthermore, the model assumes that the selection of specific existing nodes for neighbor roles (in the number equal to the maximum number of all neighbors at most) and new connections is random.


%A natural characteristic of the model is that nodes with a higher degree are more likely to participate in the interaction, in which the proactive node has at least one neighbor. Although proactive node of the interaction and its neighbors are being selected at random, high degree node has a greater chance of being selected as neighbor of the proactive node.

A natural characteristic of the model is that nodes with a higher degree are more likely to participate in an interaction in which the proactive node has at least one neighbor. Although a proactive node of the interaction and its neighbors are being selected at random, a high degree node has a greater chance of being selected as a neighbor of the proactive node.


$\lambda_1$, $\lambda_2$ and $\lambda_3$ significantly affect the density of the network. If we assume that a randomly selected interaction has, based on the corresponding distributions, $b$ neighbors of a proactive node, $n$ new nodes and $e$ nodes unconnected to the proactive node, then the number of nodes involved in this interaction (interaction size) is in Equation \ref{eq:xdef} 

\begin{equation} s = 1 + b + n + e \label{eq:xdef}
\end{equation}

and the following applies:

\begin{itemize}
	\item $n$ new nodes, which must connect to a proactive node and each other, is created.
	\item There are $b$ nodes adjacent to the proactive node which must first get connected among each other, then with $e$ nodes that are not adjacent to the proactive node (these edges may already exist prior to the interaction). Finally, they must connect with the new $n$ nodes.
	\item There are $e$ nodes not adjacent to the proactive node, which must get connected with it. Next, they must get connected among each other (these edges may already exist prior to the interaction) and $n$ new nodes.
\end{itemize}

%It follows, that the minimum and the maximum number of new connections (edges) is:

The minimum and the maximum number of new connections (edges) is in Equations \ref{eq:min} and \ref{eq:max}, respectively.

\begin{equation}	MIN = n + e + b \cdot n + e \cdot n + \frac{n \cdot (n - 1)}{2} \label{eq:min}
\end{equation}

\begin{equation} MAX = MIN + e \cdot b + \frac{b \cdot (b - 1)}{2} + \frac{e \cdot (e - 1)}{2} \label{eq:max}
\end{equation}

Thus, if for example we set $b = 2, n = 3, e = 1$ for the interaction, then:

\begin{itemize}
	\item interaction size is $s = 1 + 2 + 3 + 1 = 7$
	\item after the interaction a total of $21$ edges exist between pairs of nodes
	\item $MIN = 3 + 1 + 6 + 3 + 3 = 16$ in the case of $5$ edges existing between pairs of nodes prior to the interaction
	\item $MAX = 10 + 2 + 1 + 0 = 19$ in the case of $2$ edges existing between pairs of nodes prior to the interaction
\end{itemize}

Each of $\lambda_1$, $\lambda_2$ and $\lambda_3$ affects different property of the network generated by 3-lambda model.

%\noindent
%\noindent
%$\lambda_2$ (newbies) defines the growth rate of the network and provides a tree-like network structure, see Fig. \ref{fig:lambda2net}. To construct a network with $N$ nodes requires approximately $N/$$\lambda_2$ interactions.
%
%
%\noindent
%\noindent
%$\lambda_1$ (base/neighbors) constitutes network community structure through local connections of existing neighbors and new nodes, see Fig. \ref{fig:lambda1net}.
%
%\begin{flushright}
%
%\end{flushright}
%
%\noindent
%\noindent
%$\lambda_3$ (new connections) ensures linking of nodes that are not adjacent, thereby linking communities. The consequence is emerging of \textit{nested - core - periphery} network structure, see Fig. \ref{fig:lambda3net}.

\begin{itemize}
	\item $\lambda_2$ (newbies) defines the growth rate of the network and provides a tree-like network structure, see Fig. \ref{fig:lambda2net}. To construct a network with $N$ nodes requires approximately $N/$$\lambda_2$ interactions.
	\item $\lambda_1$ (neighbors) constitutes network community structure through local connections of existing neighbors and new nodes, see Fig. \ref{fig:lambda1net}.
	\item $\lambda_3$ (new connections) ensures linking of nodes that are not adjacent, thereby linking communities. The consequence is emerging of core-periphery network structure, see Fig. \ref{fig:lambda3net}.
\end{itemize}


%Figure \ref{fig:wholenet} shows a network with $1003$ nodes and $5594$ edges generated with parameters $\lambda_1$ = 2, $\lambda_2$ = 3, $\lambda_3$ = 0.5. A total of $347$ interactions took place. The size of nodes and strength of edges correspond to the number of interactions they took part in, the label indicates the order in which nodes were created. The network has a distinct \textit{community} and \textit{nested - core - periphery} structure. Colored $17$ communities were detected  by Louvein[REF!!] method, modularity is $0.683$.
%
%\begin{figure}[h]
%\centering
%\includegraphics[width =\columnwidth]{figures/1000-2-3-05}
%\caption{$\lambda_1$ = 2, $\lambda_2$ = 3, $\lambda_3$ = 0.5; 1003 nodes network}
%\label{fig:wholenet}
%\end{figure}

\subsection{Network Generator}
\label{sec:alg}
The network generator uses a simple algorithm which comes directly from the model description. The only extra step is setting up the initial network state. The model is memory-less, which allows working with an arbitrary initial state. For our generator we chose a complete graph with a number of nodes equal to the round of $(1 + \lambda_1 + \lambda_2 + \lambda_3)$ as the default state. Algorithm \ref{alg:1} describes the whole process of generating a network. The generated network is a connected graph; the algorithm starts with a complete graph and each interaction contains at least one existing node. In our implementation, for reasons of analysis and visualization, we store the number of interactions for each node and edge, which is not mentioned in the algorithm.

\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{number of nodes $N$, $\lambda_1, \lambda_2, \lambda_3$}
\Output{generated network $G$}
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
\SetAlgoLined
choose $s = ROUND(1 + \lambda_1 + \lambda_2 + \lambda_3)$\\
create $G = (V, E)$  as a complete graph with $s$ nodes\\

\While{$V$ has less than $N$ nodes}
{ 
  choose from $V$ randomly proactive node $A$ \\
  $b =$ number of neighbors by Poisson($\lambda_1$) ($b$ is the number of neighbors of $A$ at most) \\
  $n =$ number of newbies by Poisson($\lambda_2$)\\
  $e =$ number of new connections by Poisson($\lambda_3$)\\

  create a list $I$ with a proactive node $A$\\
  add to list $I$ $b$ randomly selected neighbors of node $A$ from $V$\\
  create $n$ new nodes, add them to $V$ and $I$\\
  add to list $I$ $e$ randomly selected not-neighbors of node $A$ from $V$ (if such nodes exist)\\

 \ForEach{pair of nodes $(V_i,V_j) \in I$}
 {
    \If{no edge $e$ between $V_i$ and $V_j$ exists}
    {
      create $e$ and add to $E$\\
    }
 }
}
%return $GN$\\

\caption{3-lambda model network generator}\label{alg:1}
\end{algorithm}


The average number of nodes in an interaction is approximately  $s = 1 + \lambda_1 + \lambda_2 + \lambda_3$. However, the average is slightly lower because the number of neighbors selected for interaction through the simulation of the Poisson distribution is limited by the actual (maximum) number of neighbors of the proactive node.

The complexity of the algorithm is $O (s^2 \cdot \frac{N}{\lambda_2})$, which is based on the fact that:

\begin{itemize}
	  \item To generate $N$ nodes requires approximately $N / \lambda_2$ interactions ($\lambda_2$ is the average number of new nodes in one interaction).
    \item The number of edges between nodes in an interaction is in quadratic relation to the number of nodes of this interaction (the interaction takes place in a complete sub-graph with $n$ nodes and $m = \frac{n * (n-1)}{2}$ edges).
\end{itemize}

The calculation of algorithm complexity does not include the complexity of the simulation of the Poisson distribution for individual \textit{lambdas} (in our case, the Knuth's algorithm with complexity $O(\lambda)$ was used).
